Predicting Progression Events in Multiple Myeloma from Routine Blood Work

The ability to accurately predict disease progression is paramount for optimizing multiple myeloma patient care. This study introduces a hybrid neural network architecture, combining Long Short-Term Memory networks with a Conditional Restricted Boltzmann Machine, to predict future blood work of affected patients from a series of historical laboratory results. We demonstrate that our model can replicate the statistical moments of the time series ($0.95~\pm~0.01~\geq~R^2~\geq~0.83~\pm~0.03$) and forecast future blood work features with high correlation to actual patient data ($0.92\pm0.02~\geq~r~\geq~0.52~\pm~0.09$). Subsequently, a second Long Short-Term Memory network is employed to detect and annotate disease progression events within the forecasted blood work time series. We show that these annotations enable the prediction of progression events with significant reliability (AUROC$~=~0.88~\pm~0.01$), up to 12 months in advance (AUROC($t+12~$mos)$~=0.65~\pm~0.01$). Our system is designed in a modular fashion, featuring separate entities for forecasting and progression event annotation. This structure not only enhances interpretability but also facilitates the integration of additional modules to perform subsequent operations on the generated outputs. Our approach utilizes a minimal set of routine blood work measurements, which avoids the need for expensive or resource-intensive tests and ensures accessibility of the system in clinical routine. This capability allows for individualized risk assessment and making informed treatment decisions tailored to a patient's unique disease kinetics. The represented approach contributes to the development of a scalable and cost-effective virtual human twin system for optimized healthcare resource utilization and improved patient outcomes in multiple myeloma care.

==> tables/forecast_performance_data.tex <==
%Transposed Version of the table above.
\begin{table*}[t]
    \centering
    \caption{Annotation performance in forecasted blood work.}
    \label{tab:forecast_performance}
    \begin{tabular}{l c c c c c}
        \toprule
        \textbf{Forecasting Horizon}  & \textbf{3 months} & \textbf{6 months} & \textbf{9 months} & \textbf{12 months} & \textbf{15 months} \\
        \midrule
        \textbf{AUROC}                & $0.78 \pm 0.02$   & $0.71 \pm 0.02$   & $0.67 \pm 0.02$   & $0.65 \pm 0.01$    & $0.62 \pm 0.02$    \\
        \textbf{AUPRC}                & $0.21 \pm 0.02$   & $0.18 \pm 0.02$   & $0.16 \pm 0.02$   & $0.15 \pm 0.03$    & $0.14 \pm 0.03$    \\
        \textbf{Sensitivity (Recall)} & $0.78 \pm 0.04$   & $0.67 \pm 0.05$   & $0.61 \pm 0.05$   & $0.59 \pm 0.05$    & $0.57 \pm 0.05$    \\
        \textbf{Specificity}          & $0.67 \pm 0.03$   & $0.68 \pm 0.03$   & $0.67 \pm 0.04$   & $0.65 \pm 0.04$    & $0.62 \pm 0.05$    \\
%        \textbf{PPV (Precision)}      & $0.17 \pm 0.01$   & $0.16 \pm 0.01$   & $0.15 \pm 0.01$   & $0.14 \pm 0.02$    & $0.13 \pm 0.02$    \\
%        \textbf{Accuracy}             & $0.68 \pm 0.03$   & $0.68 \pm 0.03$   & $0.66 \pm 0.03$   & $0.64 \pm 0.03$    & $0.62 \pm 0.04$    \\
        \bottomrule
    \end{tabular}
\end{table*}
